SpoofCeleb: Speech Deepfake Detection and SASV In The Wild

This paper introduces SpoofCeleb, a dataset designed for Speech Deepfake Detection (SDD) and Spoofing-robust Automatic Speaker Verification (SASV), utilizing source data from real-world conditions and spoofing attacks generated by Text-To-Speech (TTS) systems also trained on the same real-world data. Robust recognition systems require speech data recorded in varied acoustic environments with different levels of noise to be trained. However, current datasets typically include clean, high-quality recordings (bona fide data) due to the requirements for TTS training; studio-quality or well-recorded read speech is typically necessary to train TTS models. Current SDD datasets also have limited usefulness for training SASV models due to insufficient speaker diversity. SpoofCeleb leverages a fully automated pipeline we developed that processes the VoxCeleb1 dataset, transforming it into a suitable form for TTS training. We subsequently train 23 contemporary TTS systems. SpoofCeleb comprises over 2.5 million utterances from 1,251 unique speakers, collected under natural, real-world conditions. The dataset includes carefully partitioned training, validation, and evaluation sets with well-controlled experimental protocols. We present the baseline results for both SDD and SASV tasks. All data, protocols, and baselines are publicly available at https://jungjee.github.io/spoofceleb.

==> section/bio.tex <==
\begin{IEEEbiographynophoto}{Jee-weon Jung}~(Member, IEEE) received his PhD degree from the University of Seoul, Republic of Korea. He was a research scientist at Naver corporation and is now a Postdoctoral Research Associate at Carnegie Mellon University, USA. He was the main organizer of the SASV 2022. He has been an organizer of VoxSRC and ASVspoof challenges since 2022. His research focuses on audio anti-spoofing, speaker recognition, and other speech-related tasks. He is a Member of IEEE and ISCA.\end{IEEEbiographynophoto}


\begin{IEEEbiographynophoto}
{THIRD C. AUTHOR JR.}~(Member, IEEE), photograph and biography not available
at the time of publication.
\end{IEEEbiographynophoto}
\begin{IEEEbiographynophoto}{Xin Wang}
~(Member, IEEE) received his PhD degree from the SOKENDAI, Japan. He is a project associate professor at National Institute of Informatics, Japan. He was among the organizing team of the ASVspoof Challenges 2019 and 2021 and the VoicePrivacy initiatives in 2020 and 2022. His research focuses on speech audio generation, text-to-speech synthesis, anti-spoofing, and other speech security and private related tasks. He is a Member of IEEE.\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Ji-Hoon Kim}
~(Member, IEEE) is a PhD student in Electrical Engineering at Korea Advanced Institute of Science and Technology, Daejeon, Republic of Korea.
His main research interests include speech processing and multi-modal learning.
He received the M.S. degree in Artificial Intelligence from Korea University, Seoul, Republic of Korea.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Yuta Matsunaga}
~(Member, IEEE) received the B.E. and M.E. degrees in 2021 and 2023, respectively from the University of Tokyo, Tokyo, Japan, where he is currently working toward the Ph.D. degree. His research interests include speech synthesis, speech processing, and deep learning. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Hye-jin Shim}
~(Member, IEEE) is a postdoctoral researcher at Carnegie Mellon University, USA. She received her Ph.D. degree at the School of Computer Science from the University of Seoul in 2022. She was a postdoctoral researcher at the University of Eastern Finland before joining Carnegie Mellon University. Her research focuses on speaker verification, audio anti-spoofing, and acoustic scene classification.


\begin{IEEEbiographynophoto}{Joon Son Chung}
~(Member, IEEE) is an associate professor at Korea Advanced Institute of Science and Technology, where he is directing research in speech processing, computer vision and machine learning. He received the D.Phil. in Engineering Science from the University of Oxford. \end{IEEEbiographynophoto}


\begin{IEEEbiographynophoto}{Seyun Um}
~(Member, IEEE) received her PhD degree from the Yonsei University, Seoul, Republic of Korea.
Her research interests include emotional text-to-speech, 3D facial animation, articulatory-to-speech and retrieval augmented generation for multi-modal large language model.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Shinnosuke Takamichi}
~(Member, IEEE) received the Ph.D. degree from Nara Institute of Science and Technology, Japan. He is currently Associate Professor of Keio University, Japan. His research interest includes speech synthesis, spoken language processing, and corpus developments.  
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Shinji Watanabe}
~(Fellow, IEEE) is an associate professor at Carnegie Mellon University, USA. He received his Ph.D. (Dr. Eng.) degree from Waseda University, Japan.
His research interest includes speech recognition, speech enhancement, conversational AI, and speech/audio foundation models.
\end{IEEEbiographynophoto}
